Automatic Classification of Defective Photovoltaic Module Cells in Electroluminescence Images

Electroluminescence (EL) imaging is a useful modality for the inspection of photovoltaic (PV) modules. EL images provide high spatial resolution, which makes it possible to detect even finest defects on the surface of PV modules. However, the analysis of EL images is typically a manual process that is expensive, time-consuming, and requires expert knowledge of many different types of defects. In this work, we investigate two approaches for automatic detection of such defects in a single image of a PV cell. The approaches differ in their hardware requirements, which are dictated by their respective application scenarios. The more hardware-efficient approach is based on hand-crafted features that are classified in a Support Vector Machine (SVM). To obtain a strong performance, we investigate and compare various processing variants. The more hardware-demanding approach uses an end-to-end deep Convolutional Neural Network (CNN) that runs on a Graphics Processing Unit (GPU). Both approaches are trained on 1,968 cells extracted from high resolution EL intensity images of mono- and polycrystalline PV modules. The CNN is more accurate, and reaches an average accuracy of 88.42%. The SVM achieves a slightly lower average accuracy of 82.44%, but can run on arbitrary hardware. Both automated approaches make continuous, highly accurate monitoring of PV cells feasible.

==> tikzlibrarypageref.code.tex <==
\RequirePackage{etoolbox}

\newwrite\tikzexternalpageref@args

\newcommand\tikzexternalpageref@run[1]{%
  \immediate\write18{#1}%
}

\AtEndPreamble{%
  \tikzifexternalizing{}{%
    \def\tikzexternalpageref@perlcheck{\jobname.prc}%
    % Do not run the check if we already did check
    \IfFileExists{\tikzexternalpageref@perlcheck}{%
      % perl check file already exists
    }{%
      % Check whether perl is available by printing \def\errc{<code>} to the .prc file
      \tikzexternalpageref@run{sh -c "test -x \string\"\string$(command -v perl)\string\"; printf '\@percentchar s' \string\"\@backslashchar def\@backslashchar errc{$?}\string\"" > \tikzexternalpageref@perlcheck}%
    }%
    % TODO Check might not produce any file at all
    \IfFileExists{\tikzexternalpageref@perlcheck}{%
      \input{\tikzexternalpageref@perlcheck}%
      \ifx\errc\@undefined
        % TODO perl check did not produce any usable output (empty file)
        \PackageError{fo}{fo}{}%
      \else
        \ifdim\errc pt=\z@\else
          \PackageError{fo}{fo}{}%
        \fi
      \fi
    }{%
      % TODO warn the use the perl check cannot be run
    }%
  }%
  %
  \ifx\pgfincludeexternalgraphics@read@dpth@line\@undefined
    \PackageInfo{tikzexternalpageref}{tikz external library not loaded, not patching}%
  \else
    \long\def\pgfincludeexternalgraphics@read@dpth@line#1\pgfincludeexternalgraphics@read@dpth@line@EOI{%
        \pgfincludeexternalgraphics@read@dpth@line@getfirst#1\pgfincludeexternalgraphics@read@dpth@line@EOI
        \expandafter\ifcat\expandafter\noexpand\pgf@first\relax
            % Ah -- the first token is a control sequence. It belongs to
            % the .aux file.
            %
            \expandafter\ifx\pgf@first\pgfexternal@restore
                % if the first line in the .dpth file starts with the
                % magic string \pgfexternal@restore, the complete line
                % will be executed as-is. Example:
                % \pgfexternal@restore{\def\somevalue{1}}
                #1%
            \else
                % do NOT execute #1! many LaTeX commands don't support it (\label for example)
                \pgfutil@ifundefined{if@filesw}{%
                    % sorry, .aux file support only for latex
                }{%
                    % append to main .aux file (for forward references)
                    \if@filesw
                        {%
                        % TODO Cache results to avoid reading .dpth per line
                        \toks0={#1}%
                        % TODO Test for success/failure
                        % Start explicitly using sh since hashbang does not work under Cygwin
                        \immediate\write\tikzexternalpageref@args{\the\toks0}%
                        }%
                    \fi
                }%
            \fi
        \else% it is the depth (which is simply a number for backwards compatibility)
            \def\pgfexternaldepth{#1}%
        \fi
    }%
    %
    \def\pgfexternalreaddpth#1{%
        % Store non-executable .aux lines
        \def\tikzexternalpageref@filenameargs{#1.auxlines}%
        \immediate\openout\tikzexternalpageref@args=\tikzexternalpageref@filenameargs%
        % no \begingroup. Handle that manually:
        \edef\pgfexternalreaddpth@restore{%
            \noexpand\endlinechar=\the\endlinechar\space
            \noexpand\catcode`\noexpand\@=\the\catcode`\@\space
        }%
        %
        \def\pgfexternaldepth{0sp}%
        \def\pgfexternaltrimleft{0sp}%
        \def\pgfexternaltrimright{0sp}%
        \endlinechar=-1 % suppress white space at end
        \catcode`\@=11
        \openin\r@pgf@reada=#1.dpth
        \pgfincludeexternalgraphics@read@dpth
        %
        % We're done caching the .aux lines
        \immediate\closeout\tikzexternalpageref@args
        \if@filesw
          % Process the .aux lines
          \def\tikzexternalpageref@filename{#1.pageref}%
          \tikzexternalpageref@run{perl ./tikzlibrarypageref-protect.pl < \tikzexternalpageref@filenameargs > \tikzexternalpageref@filename}%
          %\tikzexternalpageref@run{rm \tikzexternalpageref@filenameargs}%
          \IfFileExists{\tikzexternalpageref@filename}{%
            \toks0={}%
            \input\tikzexternalpageref@filename%
            % Expand \toks0 and check whether the register is empty
            \long\edef\tikzexternalpageref@output{\the\toks0}%
            \ifx\tikzexternalpageref@output\@empty
              \PackageError{tikzexternalpageref}{tikzexternalpageref-protect.sh did not produce any usable output}{}%
            \fi
          }{%
            \PackageError{tikzexternalpageref}{Failed to \string\protect\space the .aux content. You may possibly need to compile using the -shell-escape option.}{%
              The document must be either compiled using the -shell-escape flag or you are missing the perl executable%
            }%
          }%
          % This is where the 'magic' happens: \thepage is the sole command not
          % protected by the previously executed script on the current .aux
          % line. At shipout, it will be expaned to the correct page number. Not
          % that we avoid defining the tokens in a \dpthimport macro followed by
          % call since we output the parameter numbers (hashes followed by a
          % digit) verbatim.
          \protected@write\@auxout{}{\the\toks0}%
        \fi
        % This must be done at the end
        \pgfexternalreaddpth@restore
    }%
  \fi
}

